Challenge-Response to Authenticate Drone Communications: A Game Theoretic Approach

As drones are increasingly used in various civilian applications, the security of drone communications is a growing concern. In this context, we propose novel strategies for challenge-response physical layer authentication (CR-PLA) of drone messages. The ground receiver (verifier) requests the drone to move to a defined position (challenge), and authenticity is verified by checking whether the corresponding measured channel gain (response) matches the expected statistic. In particular, the challenge is derived from a mixed strategy obtained by solving a zero-sum game against the intruder, which in turn decides its own positions. In addition, we derive the optimal strategy for multi-round authentication, where the CR-PLA procedure is iterated over several rounds. We also consider the energy minimization problem, where legitimate users want to minimize the energy consumption without compromising the security performance of the protocol. The performance of the proposed scheme is tested in terms of both security and energy consumption through numerical simulations, considering different protocol parameters, different scenarios (urban and rural), different drone altitudes, and also in the context of drone swarms.

==> figures/attackNaiveCheck.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmode=log,
xmin=0.001,
xmax=1,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$P_{\rm fa}$},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
grid,
xminorgrids,
yminorgrids,
ylabel style={font=\color{white!15!black}},
ylabel={$P_{\rm md}$},
%title={Pmd Vs Pfa},
legend style={at={(0.02,0.98)},anchor=north west,legend cell align=left, align=left, draw=white!15!black},
enlargelimits=false,title style={font=\scriptsize},xlabel style={font=\scriptsize},ylabel style={font=\scriptsize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
0.001	0.023771923576401\\
0.00143844988828766	0.0231305482351686\\
0.00206913808111479	0.0224628257550238\\
0.00297635144163132	0.0217530584905203\\
0.0042813323987194	0.0210183726704476\\
0.00615848211066027	0.0202621831811497\\
0.00885866790410082	0.0195091563142439\\
0.0127427498570313	0.0186993485854514\\
0.0183298071083244	0.0178336035381839\\
0.0263665089873036	0.0169494854335205\\
0.0379269019073225	0.0160248601407504\\
0.0545559478116852	0.0150071528996448\\
0.0784759970351461	0.0138711700577686\\
0.112883789168469	0.0126392977510026\\
0.162377673918872	0.011273210615562\\
0.233572146909012	0.00973986065961325\\
0.335981828628378	0.00797052473254218\\
0.483293023857175	0.00587742184518819\\
0.695192796177561	0.00331706345481242\\
1	0\\
};
\addlegendentry{Normal Game}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.001	0.999\\
0.00143844988828766	0.998561550111712\\
0.00206913808111479	0.997930861918885\\
0.00297635144163132	0.997023648558369\\
0.0042813323987194	0.995718667601281\\
0.00615848211066027	0.99384151788934\\
0.00885866790410082	0.991141332095899\\
0.0127427498570313	0.987257250142969\\
0.0183298071083244	0.981670192891676\\
0.0263665089873036	0.973633491012696\\
0.0379269019073225	0.962073098092677\\
0.0545559478116852	0.945444052188315\\
0.0784759970351461	0.921524002964854\\
0.112883789168469	0.887116210831531\\
0.162377673918872	0.837622326081128\\
0.233572146909012	0.766427853090988\\
0.335981828628378	0.664018171371622\\
0.483293023857175	0.516706976142825\\
0.695192796177561	0.304807203822439\\
1	0\\
};
\addlegendentry{Eve forte}

\end{axis}

\end{tikzpicture}%

==> review.tex <==
\newcounter{rcnt}
\newcounter{ccnt}

\newcommand{\newreviewernopagebreak}[1]{\vspace{5em} \setcounter{ccnt}{0}\section*{\normalsize Comments of #1}\vspace{4mm}}

\newcommand{\ThisIsTheEditor}{%\clearpage%
\vspace{-5em}\ThisIsTheEditorNoPageBreak}
\newcommand{\ThisIsTheEditorNoPageBreak}{\setcounter{ccnt}{0}\section*{\Large Comments of the Editor}\vspace{3mm}}
\newcommand{\ThisIsANewReviewerNoPageBreak}[1]{\vspace{5em} \refstepcounter{rcnt}\label{r#1}\setcounter{ccnt}{0}\section*{\Large Comments of Reviewer #1}\vspace{3mm}}
\newcommand{\ThisIsANewReviewer}[1]{%\clearpage
\vspace{-5em} \ThisIsANewReviewerNoPageBreak{#1}}


\newcommand{\edcomment}[1]{\fontsize{12}{15}\selectfont
\refstepcounter{ccnt}\label{e\arabic{ccnt}}\noindent\textbf{\boldmath\emph{Comment E.\arabic{ccnt}:} #1}\vspace{0.2cm}}
\newcommand{\refedcomment}[1]{E.\ref{e#1}}

\newcommand{\revcomment}[1]{\refstepcounter{ccnt}\label{r\arabic{rcnt}c\arabic{ccnt}}{\noindent\textbf{\boldmath\emph{Comment \arabic{rcnt}.\arabic{ccnt}:} #1}}\vspace{0.2cm}}
\newcommand{\refrevcomment}[2]{\ref{r#1}.\ref{r#1c#2}}

% \newcommand{\ouranswer}[1]{\noindent\emph{Answer:} #1\vspace{0.6cm}}
% \newcommand{\citepap}[1]{\vspace{0.33cm}\begin{minipage}{0.05\textwidth} $\phantom{A}$  \end{minipage}\begin{minipage}{0.85\textwidth}\renewcommand{\baselinestretch}{1.15}\small \emph{#1} \end{minipage}\vspace{0.3cm}}


\newlength{\ansspace}
\addtolength{\ansspace}{0.6cm}
\newcommand{\ansbreak}{\vspace{\ansspace}}

\newlength{\stdleftskip}
\addtolength{\stdleftskip}{\leftskip}
\newlength{\stdrightskip}
\addtolength{\stdrightskip}{\rightskip}
\newlength{\citeskip}
\addtolength{\citeskip}{3em}
\newcommand{\oldbaselinestretch}{1.25}

\newcommand{\setcitepapskip}{%
    \leftskip\citeskip %
    \rightskip\citeskip %
    \renewcommand{\baselinestretch}{1.15}\small%
    \vspace{0.6em}%
    \noindent%
    \fontsize{10}{12.5}\selectfont
}

\newcommand{\resetLRmargins}{%
    \leftskip\stdleftskip %
    \rightskip\stdrightskip %
    \renewcommand{\baselinestretch}{\oldbaselinestretch}\normalsize %
    \vspace{0.6em}
    \fontsize{12}{15}\selectfont
}

\newcommand{\emans}{\fontsize{12}{15}\selectfont\emph{Answer:\ }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setcounter{page}{1}
% \renewcommand{\thepage}{RL -- jmse-1713325 -- Page~\arabic{page}}

\noindent
\begin{minipage}{\linewidth}
\centering
 \vspace{5mm}
 {\huge    Response to Reviewers for manuscript\\[2mm] T-IFS-19797-2024} \\[5mm]
 {\LARGE ``Challenge-and-Response to Authenticate Drone Communications: A Game Theoretic Approach''} 
\end{minipage}

\vspace{5mm}
\noindent
\begin{minipage}{\linewidth}
    \centering   
    {\large Mattia~Piana, Francesco~Ardizzon, and Stefano~Tomasin}
\end{minipage}

\renewcommand{\baselinestretch}{\oldbaselinestretch}\normalsize

\vspace{10mm}


 \section*{\Large Summary of changes}
 \vspace{1mm}
 \fontsize{12}{14}\selectfont
 
We thank the Editor for the comments we received. These comments covered aspects that have helped us to strengthen the message and improve the clarity of the paper. We list below the most relevant changes to the manuscript.
\begin{itemize}
    \item We have reviewed the abstract to highlight the results.
    \item We added new simulations, and performance results are now provided for both urban and rural scenarios.
    \item We have included a strategy for multiple drone authentications, whose results have been reported in the new Fig. \ref{fig:pmd_pfa_swarms}.
    \item We added a sensitivity analysis on the initial map gain estimation, whose results are in the new Fig. \ref{fig: non_opt_stim}.
\end{itemize}
  \noindent  In the following, we provide detailed answers to those.
 \vspace{4mm}

 \hspace{4cm}Kind regards,

 \vspace{4mm}

 {\hspace{10cm} \large \textit{The Authors}}

\clearpage



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R   1                     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage

\ThisIsANewReviewer{1}

% Comment 1

\revcomment{The contribution is completely ok! The manuscript is as follows: In a training phase in the higher layers, Alice and Bob learn how to communicate with each other. In reality and in the presence of Trudy, Bob should minimize his error in detecting of Alice's current location based on Likelihood technique, whereas Trudy knows a lot -- something like she can span Alice's information vector. A Nash equilibrium is found for a defined zero-sum game between Bob and Trudy, and the non-convex optimisation problem is relaxed through some novel ideas; something that is completely novel, nice, and well-elaborated.} 

\emans We thank the Reviewer for the comments. We address the Reviewer's concerns below.

\ansbreak 

\revcomment{what are exactly $M_T, M_A$ and why "therefore $X \subseteq Y$" -- and what does it mean, from an information-theoretical point of view, that $X \subseteq Y$ should hold in your scheme -- although I know you have done something in II.C \& III.A} 

\emans $M_T$ and $M_A$ are the number of positions Trudy and Alice can pick, respectively. In the previous manuscript, we we let Trudy to use not only all the points available to Alice (thus the set of Trudy's points includes the set of Alice's points, in formulas $\mathcal X \subset \mathcal Y$), but also others (thus $M_T \geq M_A$) to let hes perform more effective attacks. Thanks to your comment, however, we realized that our solution works for any set of points of Alice and Trudy, thus we removed this assumption in the revised manuscript and now we only write: 

\setcitepapskip

\recalltext{al_tr_asymmetry}

\resetLRmargins


\ansbreak

\revcomment{why $M_A=M_T=15-by-15$ in your Table I} 

In the simulation results of Section \ref{sec:results}, Alice and Trudy move in an area of $420$ \si{\meter} $\times 420$ \si{\meter} and have the same positions available (if not otherwise stated). The positions are on a grid of 15 points on the $x$ and $y$ axes (thus the notation $15 \times 15$). 


\setcitepapskip

\recalltext{grid_desc}

\resetLRmargins


\ansbreak

\revcomment{In "The energy consumed by Alice to move from position ... traveling on a straight line": Why a straight line? Why a constant and time-independent v -- velocity?}

\emans We considered a straight-line movement as this minimizes the traveled distance, and thus also the consumed energy.
Specifically concerning the movement model, we ignored the acceleration as the distance needed for the drone to reach maximum velocity is much lower than the one between two adjacent points on the grid, i.e., \SI{15}{\meter}, in our simulation scenario. Note that, even including acceleration, the energy spent by the drone to travel distance $d$ is a linear function of $d$ plus a constant bias due to the energy spent by the drone to reach the maximum velocity. Thus, to minimize the energy consumption, we would still need to minimize $d$. 

To avoid making the model too complex, we focus on a linear energy model. Still, we agree with the Reviewer that both points should be mentioned in the paper. Thus, we updated the manuscript by introducing the following two sentences:

\setcitepapskip

\recalltext{droneEnergy1}

\resetLRmargins

and

\setcitepapskip

\recalltext{droneEnergy2} 

\resetLRmargins
\ansbreak


\revcomment{ In (37-38): this is due to the basis of the zero-sum-game, isn't it?}

\emans Yes, exactly. Equation \eqref{eq:maximin} and \eqref{eq:minimax} define the maximin and minimax problems, which, for the theory of zero-sum games, lead to an equivalent solution. To make this point clearer, we modified the manuscript by adding the following sentence:

\setcitepapskip

\recalltext{zero_sum_clar}
\textcolor{blue}{$$ 
u_{\rm T, \min}^{\star}=\min_{\bm{a}}\max_{\bm{e}}u_{\rm T}(\bm{a},\bm{e}).
$$}

\resetLRmargins
and providing the following references to the two formulas:


\setcitepapskip
\textcolor{blue}{
From the minimax theorem \cite{v1928theorie}, we have
$$        \bm{e}^\star = \bm{e}_{\rm max} = \bm{e}_{\rm min}, \quad u^{\star} = u_{\rm T, \min}^{\star} = u_{\rm T, \max}^{\star}\,\,
$$ }
\recalltext{zero_sum_clar_2}

\resetLRmargins

\ansbreak

\revcomment{why and how (42) is a dual for (26) as your index-extracting joint probability can be a conditional one -- conditioning to Trudy, something that may create any affine region in your space area -- although you declare that (42) is non-convex, relaxing it to your novel things}


\emans  We are sorry for the misunderstanding, but \eqref{eq:opt_pfa_dist} and \eqref{eq:opt_NE} are equivalent problems, not dual. To clarify the equivalence, we have added the following paragraph before \eqref{eq:opt_NE}:

\setcitepapskip


\recalltext{eq_complicata}

{\color{blue} 
 $\begin{aligned}
        \bm{A}^\star=
        {\rm arg} \min_{\bm{A}} \;  \hspace{-2mm} &\sum_{\mathcal{I}=\{i_1,\ldots,i_N\}}  \left[\sum_{n=1}^{N-1} d_{i_n,i_{n+1}} \right] p_{\mathcal I}(\mathcal{I},\bm{A}) \\      
        \textrm{s.t.} \;\;& \forall i \in 1, \ldots, M_{\rm A} \,, \forall n:  \\
       \quad & u^{\star}\mathds{1} \leq  -\bm{P}^T \bm{a}(i,n) \hspace{0.5cm} \\
        & \sum_{i'=1}^{M_{\rm A}} a_{i'}(i,n)= 1, \quad \bm{a}(i,n) \geq \bm{0}. \\
        \end{aligned}
 $
}

\resetLRmargins

About the convexity of the problem, we note that the probability in the objective function is obtained as a product of the variables, providing a non-convex function. To explain it better we added the following sentence after the problem statement:

\recalltext{commento_1.5}
\ansbreak

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R  2                     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\ThisIsANewReviewer{2}


\revcomment{The paper, "Challenge-and-Response to Authenticate Drone Communications: A Game Theoretic Approach", explores the development of a novel physical layer authentication (PLA) strategy for drone communications using a challenge-and-response mechanism. By modeling the interaction between a legitimate drone (Alice), a verifier (Bob), and an intruder drone (Trudy) as a zero-sum game, the authors propose methods for optimal challenge and response distributions to enhance authentication. The paper introduces energy-efficient approaches for challenge generation and evaluates their performance through simulations in realistic channel models. While the work provides significant insights into PLA mechanisms for drones, some areas warrant further clarification and elaboration.}

\emans We thank the Reviewer for the comments. We address the Reviewer's concerns below.

\ansbreak

\revcomment{The energy minimization strategies rely on simplified movement and energy consumption models. A more detailed consideration of drone dynamics, such as acceleration and environmental factors, would make the analysis more realistic.}


\emans  While we agree with the Reviewer that it may be interesting to include a more detailed drone model, we recall that our work focuses on the communication and its exploitation to develop the proposed CR-PLA solution. Thus, we aim to describe this solution and capture its main elements for security and communication, leaving the details of a more specific energy model that is specific to individual vehicles for specific projects or studies. 
From this perspective, we then show that it is possible to find a solution that reduces the drone's traveled distance (thus the consumed energy due to the movements), keeping the desired security level. 
Specifically concerning the movement model, we ignored the acceleration as the distance needed for the drone to reach maximum velocity, whose typical values are much lower than the tile size, which in our case is \SI{15}{\meter}. Even including acceleration, the energy spent by the drone to travel a distance $d$ is still a linear function of $d$ plus a constant bias. Thus, to minimize the energy consumption, we would still need to minimize just $d$. 
We added this consideration in the updated version of the manuscript:

\setcitepapskip

\recalltext{droneEnergy2}

\resetLRmargins


\ansbreak

\revcomment{While shadowing effects are modeled, the correlation between path loss and shadowing under different environmental conditions (e.g., urban versus rural) could be explored to generalize the results.}


\emans We agree with the Reviewer that an extension to different environments is necessary to generalize the results. We extended the simulations and added to Fig. \ref{fig: pmd_pfa_complete} and Fig. \ref{fig:pmd_pfa_swarms} lines corresponding to a shadowing standard deviation of $\sigma_{(s)_{\rm dB}}=\SI{6}{\decibel}$ that is suitable for rural environments according to~\cite{chandrasekharan2015propagation}. We show that our protocol is effective even in rural areas, yet with a slightly worse performance than in urban environments: this is expected, as a lower shadowing variance leads to worse performance, as pointed out in Section \ref{subsec: pla_param}. In addition to enriching Fig. \ref{fig: pmd_pfa_complete} and \ref{fig:pmd_pfa_swarms}, we also modified the manuscript as follows:


\setcitepapskip

\recalltext{new variance}

\resetLRmargins

We also added the following comment on Fig. 3:


\setcitepapskip

\recalltext{fig3comm}

\resetLRmargins
 

and the following comment on Fig. 7:



\setcitepapskip

\recalltext{fig7comm}

\resetLRmargins
  
\ansbreak

\revcomment{The paper identifies Nash equilibria (NE) strategies for the zero-sum game but does not discuss how these equilibria might shift under dynamic or non-ideal conditions, such as partial knowledge by Bob or Trudy.}


\emans We thank the Reviewer for the comment. We investigated how the performance might shift under non-ideal conditions in Section \ref{sec:results}. In fact, in Section \ref{par:comparison}, we show what happens if Bob adopts a strategy that chooses uniformly over the gains (i.e., he deviates from the \ac{ne}), as in the literature. We studied what happens if Trudy is aware of this, and in this case, she can perform the BAUD attack in Fig. \ref{fig:non_opt} (which is the best attack against the uniform distribution), leading to a $P_{\rm md}$ almost 10 times bigger than the \ac{ne}. We also studied the case where both Trudy and Bob play uniformly (US strategy in Fig. \ref{fig:non_opt}). In this case, the performance is between the optimal \ac{ne} and the BAUD. 

Moreover, in the revised manuscript, we added Fig. \ref{fig: non_opt_stim}, which addresses your next comment and provides performance for an imperfect channel knowledge by Bob in the first phase (finite $K_{\rm est}$). If Bob does not take into account this imperfection, he deviates from the \ac{ne} and Trudy can exploit this to design better attacks. This addition is better described in the next point of this answer to review comments.

\setcitepapskip

%\recalltext{}

\resetLRmargins

\ansbreak

\revcomment{The assumption of perfect channel gain estimation ($K \rightarrow \infty$) during the setup phase is unrealistic for practical implementations. A sensitivity analysis for finite $K$ values would enhance the robustness of the findings.}


\emans We agree with the Reviewer that $K \rightarrow \infty$ is unrealistic, and a sensitivity analysis is useful. To this end, we updated the manuscript with a paragraph investigating this issue and added the new Fig. \ref{fig: non_opt_stim}, which demonstrates that with a reasonable amount of pilots we achieve the same performance as $K \rightarrow \infty$. In particular, we considered both the case in which both Bob and Trudy update their strategies, taking into account the imperfect channel estimation, and the case in which Bob only updates the threshold for detection (without changing the movement strategy) and Trudy takes advantage of this by updating her strategy. This last setting aims at providing results on imbalanced knowledge and assumptions by the agents. Lastly, we also compared the obtained performance with the optimal case of $K_{\rm est} = \infty$. 

We updated the manuscript with the following comment to the new scenario and the new figure:

\setcitepapskip

\recalltext{Sensitivity}

\resetLRmargins

\ansbreak

\revcomment{The computational complexity of the multi-round NE optimization is briefly mentioned. A comparative evaluation of its scalability for large grids or multiple drones would be beneficial.}


\emans We thank the Reviewer for this comment. Considering the multiple \ac{ne} problem for the minimization of the \ac{md} over multiple rounds, i.e., without distance minimization in mind, the complexity actually does not scale with the number of rounds, as proven in Theorem \ref{th:trudyDinamic}. We clarified this in the paper by adding the following sentence,

\setcitepapskip

\recalltext{complexity}

\resetLRmargins

Concerning the computational complexity of problems \eqref{eq:opt_fa_sec} and \eqref{eq:opt_problem_distance}, we provided more details in the updated version of the manuscript by adding the following sentences. 

\setcitepapskip

\recalltext{complexityDistance}

\resetLRmargins
and

\setcitepapskip

\recalltext{complexity single ne new}

\resetLRmargins


Finally, specifically targeting the multiple drone scenarios, we provided new results in Section~\ref{subsec: pla_param}, where we considered a scenario where Alice and Trudy both control a swarm of two drones, placed at different altitudes. Fig.~\ref{fig:pmd_pfa_swarms} reports the results of the simulations, showing that, indeed, the proposed approach scales with the number of drones as the \ac{md} decreases by a factor of 10 going from 1 to $N_\mathrm{sw} =2$ drones.

\ansbreak

\revcomment{The abstract includes excessive technical detail that could be simplified to highlight the contributions and key results more effectively.}


\emans We thank the Reviewer for the suggestion. We have revised the abstract to highlight the contributions of our paper. 

\setcitepapskip

%\recalltext{}

\resetLRmargins

\ansbreak

\revcomment{The proposed method is evaluated primarily for urban environments. Incorporating evaluations for scenarios like open fields, maritime settings, or dynamic drone swarms would broaden its applicability.}

\emans We agree with the Reviewer that an extension to different environments is necessary to generalize the results. We extended the simulations and added to Fig.~\ref{fig: pmd_pfa_complete} and Fig.~\ref{fig:pmd_pfa_swarms} lines corresponding to a shadowing standard deviation of $\sigma_{(s)_{\rm dB}}=\SI{6}{\decibel}$ that is suitable for rural environments according to~\cite{chandrasekharan2015propagation}. See your point 2.3 for more details. 


Moreover, we also investigated how the protocol performs with multiple drones, thus, we added a remark on the System Model section:

\setcitepapskip

\recalltext{multi drones}

\resetLRmargins

We performed new simulations for a multi-drone scenario whose results are in Fig. \ref{fig:pmd_pfa_swarms}, and we added the following new paragraph in Section \ref{sec:results}:  

\setcitepapskip

\recalltext{multipleDrones}

\resetLRmargins

\ansbreak

\revcomment{The paper could benefit from citing works such as "Federated Learning for Drone Authentication" "Enabling drones in the internet of things with decentralized blockchain-based security", which explores complementary approaches to authentication in drone networks.}

\emans We thank the Reviewer for the suggestions. The work 
\textit{A. Yazdinejad, R. M. Parizi, A. Dehghantanha, and H. Karimipour, “Federated learning for drone authentication,” Ad Hoc Netw., vol. 120, p. 102574, Sept. 2021. } is now among the references. On the other hand, we left out the second-mentioned work as it explores crypto solutions, which are out of the scope of our paper.  

\setcitepapskip

%\recalltext{}

\resetLRmargins

\ansbreak

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R  3                     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\ThisIsANewReviewer{3}


\revcomment{The authors have to confirm this paper was not published earlier. Please check the https://arxiv.org/pdf/2410.00785}

\emans We confirm that the paper has not been published earlier. The linked paper is actually the preprint version of the submitted article. 

\setcitepapskip

%\recalltext{}

\resetLRmargins

\ansbreak

\clearpage




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                     R E V I E W E R 4                     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\ThisIsANewReviewer{4}


\revcomment{Completeness of the Game Model – In a zero-sum game, Bob's gain is Trudy's loss, and vice versa. If Bob’s cost (energy usage in this case) influences his strategy— as suggested by his choice of the cheapest Nash Equilibrium — then Trudy must consider this influence when selecting her own strategy. Even if the cost is not directly included in Trudy’s utility function, it indirectly shapes her decision-making by influencing Bob’s behavior. Excluding cost from the payoff matrix misrepresents the true strategic interaction since Trudy’s optimal strategy depends on anticipating Bob’s actions, and Bob’s cost is a key determinant of those actions. Therefore, the cost should be incorporated into the model, even if only implicitly through its effect on Bob's choices.}

\emans We thank the Reviewer for this comment. We agree that we could have included energy in Bob's payoff function. However, this approach would have caused two major problems: a) mixing the two objectives (security and energy reduction) is problematic because they are measured by incomparable metrics (misdetection probability and energy); b) the resulting game would not be zero-sum, leading to a complex analysis of Nash equilibria. Therefore, we decided to prioritize the security objective by considering only NEs obtained by minimizing the misdetection probability at Bob, which yields a zero-sum game. Among all possible NEs, we then choose the one that minimizes the energy (or, equivalently, the distance traveled). Note that selecting a particular NE does not affect the solution security, nor can it be used to the attacker's advantage. To make this point clearer, we have added the following sentence:

\setcitepapskip

\recalltext{dist among ne}

\resetLRmargins

\ansbreak





\revcomment{Security of Initial Position \& Quantum Resistance Assumption – The paper does not explain how Alice and Bob securely agree on the initial position, which is critical for authentication. If cryptographic methods are used, they may be vulnerable to quantum attacks, contradicting the claim of quantum resistance.}

\emans We thank the Reviewer for this comment. We agree that the transmission of the initial position is a critical point in the proposed algorithm. However, there are various solutions that may be employed to secretly transmit the initial position, while still maintaining the overall protocol secure against quantum attacks.
For instance, assuming that Alice and Bob share a (short) key (e.g., this key sharing can be done at the moment of drone Alice's deployment), Bob can securely transmit the initial position using a one-time pad encryption. This solution is resistant to quantum attacks. Alternatively, it may be possible to use other information-theoretic (quantum-resistant) secure solutions based, for instance, on physical security itself (e.g., wiretap coding).  To make this point clearer, we updated the paper briefly reporting such considerations, as follows: 

\setcitepapskip

\recalltext{QuantumSecureInitPos}

\resetLRmargins

\ansbreak


\revcomment{Observability of Alice’s Location \& Violation of Authentication Best Practices – The method assumes Trudy cannot observe Alice’s position. However, if she can, the authentication can be bypassed. Good authentication practices do not rely on hiding observable factors, making this a potential security weakness.}

\emans We thank the Reviewer for the comment. We agree that getting information on the location of the drone through cameras can provide information useful for more effective attacks. However, at the state of the art, the localization of drones with ground devices is rather coarse and can be performed with a precision of a few meters, and in some (best) cases tens of centimeters, depending on the altitude of the drone, as discussed in the survey \cite{9409835}. Yet, none of the proposed methods is applicable in our scenario as they require either multiple transmitters/receivers or a super-resolution 3D multipath model of the environment. Concerning the use of visual data, solutions typically consider distributed systems to enhance the visual diversity, but still achieve a limited localization accuracy ($\SI{8}{\meter}$ in \cite{Srigrarom2021Multi-camera}). Moreover, the attacker in our scenario is a movable device, thus the performance would be even worse than the aforementioned works. Note also that the tracking must be timely so that the attacker knows the exact position when the drone is transmitting. Therefore, although we recognize the potential for more sophisticated attacks that should be investigated in the future, the proposed authentication framework is useful in various applications. To take into account your observation, we have modified the manuscript as follows: 

\setcitepapskip

\recalltext{AlternativeSharing}

\resetLRmargins

%\hl{DISCUSS} Finally, we remark that it is common in physical layer security to make assumptions on the channel/observability. For instance, all machine learning \ac{pla} schemes assume having an a priori secure dataset, which is later used the train the classifier/detector. Another common assumption in physical layer confidentiality schemes, e.g., wiretap coding, the legitimate party is supposed to have a better channel (e.g., better SNR) than the adversary. 



\ansbreak





\revcomment{Scalability Concerns – The paper does not discuss how the approach scales in multi-drone or large-scale deployments, which could limit its practical applicability.}


\emans We agree with the Reviewer that a more in-depth study on the scalability with multiple drones can enhance the applicability of the protocol. To this end, we first mentioned in the System Model the possibility of having multiple drones:

\setcitepapskip

\recalltext{multi drones}

\resetLRmargins

\noindent and then performed a new analysis in which we consider a scenario where Alice and Trudy maneuver two drones each. To avoid any possible collision, Alice set the drones to fly at different altitudes. Additionally, Alice, to avoid introducing any degree of correlation that the attacker may exploit, flies her drones to move independently from one another. 
In turn, to maximize her chance of success, Trudy sets each of her own drones to fly independently but at the same altitudes as Alice's drones. As each Alice-Trudy pair of drones plays independently from the others, we can split the game into two separate games, each solved using \eqref{eq:opt_problem}. Leveraging on the independence, we use test \eqref{eq:LLTTest} considering $N = 2$, as the shadowing maps and thus reference gains are known.
We remark that games played at different rounds are performed on the same shadowing map, while games played at the same time but at different altitudes are played on a different shadowing map. Thus, while in the $N=2$ round case, the same strategy can be used in both games, for the two drones (single round) scenario, a new strategy has to be computed for each drone pair. 

We took into account the Reviewer's comment, added Fig. \ref{fig:pmd_pfa_swarms} showing the performance of the protocol in a the multi-drone scenario, and modified the manuscript as follows:

\setcitepapskip

\recalltext{multipleDrones}

\resetLRmargins

\ansbreak


==> tikz_folder/old_tikz/pmd_pfa_full.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{RGB}{228,26,28}%
\definecolor{mycolor2}{RGB}{55,126,184}%
\definecolor{mycolor3}{RGB}{77,175,74}%
%
\begin{tikzpicture}[ every plot/.style={thick}]

\begin{axis}[%
width=\fwidth,
height=0.7\fheight,
at={(0.758in,0.481in)},
scale only axis,
xmode=log,
xmin=0.0001,
xmax=1,
xminorticks=true,
xlabel={$P_{\rm fa}$},
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
ylabel={$P_{\rm md}$},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left,at={(0.03,0.5)},anchor=west}
]
\addplot [color=mycolor1,thick, mark=square, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0.0001	0.17690812442379\\
0.000562341325190349	0.152552737252718\\
0.00316227766016838	0.130612499354946\\
0.0177827941003892	0.106006398106752\\
0.1	0.074820808144174\\
0.2825	0.0497928100070259\\
0.455	0.0349094719333417\\
0.6275	0.0227772396593468\\
0.8	0.0119201513645131\\
0.9	0.00591633388468498\\
0.92475	0.00444734873723599\\
0.9495	0.00298230980333395\\
0.97425	0.0015199243392757\\
0.999	5.88711445456635e-05\\
};
\addlegendentry{$\sigma_{(s)_{\rm dB}}=10$ \si{\decibel}}

\addplot [color=mycolor2,thick, mark=triangle, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.0001	0.133962725311744\\
0.000562341325190349	0.11632760944939\\
0.00316227766016838	0.098480568561753\\
0.0177827941003892	0.0794082662974354\\
0.1	0.0568520408705434\\
0.2825	0.0382868048132908\\
0.455	0.0269925564526704\\
0.6275	0.0176743813882766\\
0.8	0.00926804674759431\\
0.9	0.00460267165122591\\
0.92475	0.00346014269643612\\
0.9495	0.00232045126711375\\
0.97425	0.00118265005041708\\
0.999	4.58123449551616e-05\\
};
\addlegendentry{$\sigma_{(s)_{\rm dB}}=13$ \si{\decibel}}

\addplot [color=mycolor3,thick, mark=o, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0.0001	0.116489135216096\\
0.000562341325190349	0.103035038656635\\
0.00316227766016838	0.0872482712763825\\
0.0177827941003892	0.071578899893607\\
0.1	0.0510339113072291\\
0.2825	0.0344102287866878\\
0.455	0.0242771060780296\\
0.6275	0.0159054142399764\\
0.8	0.00834383512701747\\
0.9	0.00414417832627431\\
0.92475	0.00311552048429459\\
0.9495	0.00208936273265817\\
0.97425	0.00106488674304904\\
0.999	4.12482120844551e-05\\
};
\addlegendentry{$\sigma_{(s)_{\rm dB}}=16$ \si{\decibel}}

\addplot [color=mycolor3,thick, only marks,mark=*, mark options={solid, black,scale=0.4}]
  table[row sep=crcr]{%
0.0001	0.177494\\
0.000562341325190349	0.152102\\
0.00316227766016838	0.129976\\
0.0177827941003892	0.104964\\
0.1	0.074928\\
0.2825	0.049656\\
0.455	0.034834\\
0.6275	0.02288\\
0.8	0.011852\\
0.9	0.005896\\
0.92475	0.00451\\
0.9495	0.003026\\
0.97425	0.00155\\
0.999	5.4e-05\\
};
\addlegendentry{Simulated}

% \addplot [color=mycolor5, only marks, mark=x, mark options={solid, black}, forget plot]
%   table[row sep=crcr]{%
% 0.0001	0.133844\\
% 0.000562341325190349	0.116358\\
% 0.00316227766016838	0.097754\\
% 0.0177827941003892	0.079788\\
% 0.1	0.057508\\
% 0.2825	0.038362\\
% 0.455	0.027134\\
% 0.6275	0.01769\\
% 0.8	0.00955\\
% 0.9	0.004574\\
% 0.92475	0.003388\\
% 0.9495	0.002412\\
% 0.97425	0.001138\\
% 0.999	3.8e-05\\
% };
\addplot [color=mycolor3, only marks, mark=*, mark options={solid, black,scale=0.4}, forget plot]
  table[row sep=crcr]{%
0.0001	0.115204\\
0.000562341325190349	0.102598\\
0.00316227766016838	0.087276\\
0.0177827941003892	0.072398\\
0.1	0.050526\\
0.2825	0.034568\\
0.455	0.024682\\
0.6275	0.015994\\
0.8	0.008376\\
0.9	0.004234\\
0.92475	0.003046\\
0.9495	0.002198\\
0.97425	0.001146\\
0.999	4.8e-05\\
};
\end{axis}
\end{tikzpicture}%
